Parallel Minimum Cuts in $O(m \log^2(n))$ Work and Low Depth

We present a randomized $O(m \log^2 n)$ work, $O(\text{polylog } n)$ depth parallel algorithm for minimum cut. This algorithm matches the work bounds of a recent sequential algorithm by Gawrychowski, Mozes, and Weimann [ICALP'20], and improves on the previously best parallel algorithm by Geissmann and Gianinazzi [SPAA'18], which performs $O(m \log^4 n)$ work in $O(\text{polylog } n)$ depth. Our algorithm makes use of three components that might be of independent interest. Firstly, we design a parallel data structure that efficiently supports batched mixed queries and updates on trees. It generalizes and improves the work bounds of a previous data structure of Geissmann and Gianinazzi and is work efficient with respect to the best sequential algorithm. Secondly, we design a parallel algorithm for approximate minimum cut that improves on previous results by Karger and Motwani. We use this algorithm to give a work-efficient procedure to produce a tree packing, as in Karger's sequential algorithm for minimum cuts. Lastly, we design an efficient parallel algorithm for solving the minimum $2$-respecting cut problem.

==> approx-min-cut.tex <==
\section{A Parallel Constant-Factor Minimum Cut Approximation}\label{sec:const-approx}

  Step one of Karger's procedure for producing a tree packing is to compute a constant-factor approximation to the minimum cut, which is then used to derive the sampling probability for constructing a sparse skeleton. In this section, we will derive an algorithm for a constant-factor approximate minimum cut that runs in $O(m \log^2(n))$ work and $O(\polylog(n))$ depth. Karger and Motwani~\cite{karger1994derandomization} give an algorithm that runs in $O(m^2/n)$ work and $O(\polylog(n))$ depth. We achieve our bounds by improving Karger's algorithm and speeding up several of the components. Specifically, we use the following combination of ideas, new and old.
  \begin{enumerate}[leftmargin=*]
    \setlength\itemsep{0em}
    \item We extend a $k$-approximation algorithm of Karger~\cite{karger1993global} to work in parallel, allowing us to produce an $O(\log(n))$-approximate minimum cut in low work and depth
    \item The $\log(n)$-approximate minimum cut allows us to make $O(\log\log(n))$ guesses of the minimum cut such that at least one of them is a constant-factor approximation
    \item We use a faster sampling technique for producing Karger's skeletons for weighted graphs. This is done by transforming the graph into a graph that maintains an approximate minimum cut but has edge weights each bounded by $O(m \log(n))$, and then using binomial random variables to sample all of the multiedges of a particular edge at the same time, instead of separately.
    \item We show that the parallel sparse $k$-certificate algorithm of Cheriyan, Kao, and Thurimella~\cite{cheriyan1993scan} for unweighted graphs can be modified to run on weighted graphs
    \item We show that Karger and Motwani's parallelization of Matula's algorithm can be modified to run on weighted graphs
  \end{enumerate}
  
  \noindent We will use the following result due to Karger.

  \begin{definition}[$p$-skeleton of a graph]
    Given an unweighted graph $G$ and a probability $p$, the \emph{skeleton} $G(p)$ consists of the vertices of $G$ and a random subset of the edges of $G$, each sampled with probability $p$.
  \end{definition}

  \begin{lemma}[Karger~\cite{karger1995random}]\label{lemma:sampling_verified}
    With high probability, if $G(p)$ is constructed and has minimum cut $\hat{c} = \Omega(\log(n)/\varepsilon^2)$ for $\varepsilon \leq 1$, then the minimum cut in $G$ is $(1 \pm \varepsilon)\hat{c}/p$.
  \end{lemma}
  
  \subsection{Parallelising the $k$-approximation algorithm} 
 Karger describes an $O(m n^{2/k} \log(n))$ time sequential algorithm for finding a cut in a graph within a factor of $k$ of the optimal cut~\cite{karger1993global}.  
Karger's algorithm works by randomly selecting edges to contract with probability proportional to their weight until a single vertex remains, and keeping track of the component with smallest incident weight (not including internal edges) during the contraction.  This relies on the following Lemma.
  \begin{lemma}[Karger~\cite{karger1993global}]\label{lem:approx-trial}
    Given a weighted graph with minimum cut $c$, with probability $n^{-2/k}$, the meta-vertex with minimum incident weight encountered during a single trial of the contraction algorithm implies a cut of weight at most $kc$.
  \end{lemma}
\noindent Running $O(n^{2/k}\log(n))$ rounds yields a cut of size at most $kc$ w.h.p.
Here we show how to parallelize Karger's algorithm using our batched mixed operations algorithm yielding the following result:
  \begin{lemma}\label{lem:k-approx}
    For a weighted graph, a cut within a factor of $k$ of the minimum cut can be found w.h.p.\ in $O(m n^{2/k} \log^2(n))$ work 
    and polylogarithmic depth. 
  \end{lemma}

  \noindent Karger shows how to parallelize picking the (weighted) random permutation of the edges with $O(m \log^2 (n))$ work.  It can easily slightly modified to improve the bounds by a logarithmic factor as follows. The algorithm selects the edges by running a prefix sum over the edge weights.  Assuming a total weight of $W$, it then picks $m$ random integers up to $W$, and for each uses binary search on the result of the prefix sum to pick an edge.  This process, however, might end up picking only the heaviest edges.  Karger shows that by removing those edges the total weight $W$ decreases by a constant factor, with high probability.  Since the edges can be preprocessed to be polynomial in $n$ (see below), repeating for $\log(n)$ rounds the algorithm will select all edges in the appropriate weighted random order.  Each round takes $O(m \log(n))$ work for a total of $O(m \log^2 (n))$ work.  

Replacing the binary search in Karger's algorithm with a sort of the random integers and merge into the result of the prefix sum yields an $O(m \log (n))$ work randomized algorithm.  In particular $m$ random numbers uniformly distributed over a range can be sorted in $O(m)$ work and $O(\log (n))$ span by first determining for each number which of $m$ evenly distributed buckets within the range it is in, then sorting by bucket using an integer sort~\cite{RR89} and finally sorting within buckets.

The more interesting part to parallelize is identifying the component with smallest incident weight during the contraction process.  Identifying the edges that are contracted is easy using a minimum spanning tree over the position on which the edge is selected, but keeping track of the smallest incident weight of a component is somewhat trickier.
% Here we show how to parallelize the process using batched mixed operations. Lemma~\ref{lem:approx-trial} says that a single trial of the contraction algorithm will encounter a $k$-approximate cut with probability $n^{-2/k}$, and hence by testing $n^{2/k} \log(n)$ random contractions, we will find a $k$-approximate cut w.h.p.  To parallelize this algorithm, it suffices to show that we can determine the smallest-degree meta-vertex that arises during a single contraction process efficiently in parallel.
    To achieve this, we use our batched mixed operations framework from Section~\ref{sec:batched-mixed-ops}. In Appendix~\ref{sec:batch-component-weight}, we show that that the following operations have a \simpleRC{} implementation
and therefore are applicable to our method.

\begin{itemize}[leftmargin=*]
  \setlength\itemsep{0em}
  \item \textproc{SubtractWeight}($v$, $w$): Subtract weight $w$ from vertex $v$
  \item \textproc{JoinEdge}($e$): Mark the edge $e$ as ``joined''
  \item \textproc{QueryWeight}($v$): Return the weight of the connected component containing the vertex $v$, where the components are induced by the joined edges 
\end{itemize}
  
  \noindent With this tool, we can simulate the contraction process, 
%recalling that we treat a weighted graph conceptually (but not in implementation) like an unweighted multigraph with multiplicity, 
and determine the minimum incident weight of a component as follows:
  \begin{enumerate}[leftmargin=*]
    \setlength\itemsep{0em}
    \item\label{step:mst-for-approx} Compute an MST with respect to the random edge ordering, where a heavier weight indicates that an edge contracts later
    \item\label{step:heaviest-edge-for-approx} For each edge $(u,v) \in G$, determine the heaviest edge in the MST on the unique $(u,v)$ path
    \item\label{step:batch-component-weight} Construct a vertex-weighted tree from the MST, where the weights are the total
incident weight on each vertex in $G$. For each edge $(u,v)$ in the MST in contraction order:
    \begin{itemize}[leftmargin=*]
      \item Determine the set of edges in $G$ such that $(u,v)$ is the heaviest edge on its MST path. For each such edge identified, \textproc{SubtractWeight} from each of its endpoints by the weight of the edge
      \item Perform \textproc{JoinEdge} on the edge $(u,v)$
      \item Perform \textproc{QueryWeight} on the vertex $u$
    \end{itemize}
  \end{enumerate}
  
\noindent Observe that the weight of a component at the point in time when it is queried is precisely the total weight of incident
edges (again, not including internal edges). Taking the minimum over the initial degrees and all query results therefore yields the desired answer.


Step~\ref{step:mst-for-approx} takes $O(m\log(n))$ work and $O(\log^2(n))$ depth to compute the random edge permutation using Karger's technique~\cite{karger1993global}, and $O(m)$ work and $O(\log(n))$ depth to run a parallel MST algorithm~\cite{karger1995randomized}. Step~\ref{step:heaviest-edge-for-approx} takes $O(m \log(n))$ work and $O(\log(n))$ depth using RC trees~\cite{acar2005experimental,acar2020batch}, and Step~\ref{step:batch-component-weight} takes $O(m \log(n))$ work and $O(\log^2(n))$ depth using our batched mixed operations algorithm (Theorem~\ref{theorem:batch}). 

Based on Lemma~\ref{lem:approx-trial}, trying $O(n^{2/k}\log(n))$ random contractions yields the result of Lemma~\ref{lem:k-approx}. Setting $k = \log (n)$ then gives a $\log (n)$ approximation in $O(m \log^2 (n))$ work and $O(\log^2(n))$ depth.
  
  
  % \begin{lemma}\label{lem:logn-approx}
  %     A cut within a factor $\log(n)$ of the minimum cut can be found w.h.p.\ in $O(m \log^2(n))$ work and $O(\log^2(n))$ depth.
  %   \end{lemma}
  
  \subsection{Transformation to bounded edge weights} For our algorithm to be efficient, we require that the input graph has small integer weights. Karger~\cite{karger1995random} gives a transformation that ensures all edge weights of a graph are bounded by $O(n^5)$ without affecting the minimum cut by more than a a constant factor. For our algorithm $O(n^5)$ would be too big, so we design a different transformation that guarantees all edge weights are bounded by $O(m \log(n))$, and only affects the weight of the minimum cut by a constant factor.
  
  \begin{lemma}\label{lem:low-weight-transform}
    There exists a transformation that, given an integer-weighted graph $G$, produces an integer-weighted graph $G'$ no larger than $G$, such that $G'$ has edge weights bounded by $O(m\log(n))$, and the minimum cut of $G'$ is a constant-approximate minimum cut in $G$.
  \end{lemma}
  \begin{proof}
    Let $G$ be the input graph and suppose that the true value of the minimum cut is $c$. First, we use Lemma~\ref{lem:k-approx} to obtain a $O(\log(n))$-approximate minimum cut, whose value we denote by $\tilde{c}$ ($c \leq \tilde{c} \leq c \log(n)$). We can contract all edges of the graph with weight greater than $\tilde{c}$ since they can not appear in the minimum cut. Let $s = \tilde{c} / (2m \log(n))$. We delete (not contract) all edges with weight less than $s$. Since there are at most $m$ edges in any cut, this at most affects the value of a cut by $sm = \tilde{c} / (2 \log(n)) \leq c/2$. Therefore the minimum cut in this graph is still a constant factor approximation to the minimum cut in $G$.
    
    Next, scale all remaining edge weights down by the factor $s$, rounding down. All edge weights are now integers in the range $[1, 2m \log(n)]$. This is the transformed graph $G'$. It remains to argue that the value of the minimum cut is a constant-factor approximation. First, note that the scaling process preserves the order of cut values, and hence the true minimum cut in $G$ has the same value in $G'$ as the minimum cut in $G'$. Consider any cut in $G'$, and scale the weights of the edges back up by a factor $s$. This introduces a rounding error of at most $s$ per edge. Since any cut has at most $m$ edges, the total rounding error is at most $sm \leq c/2$. Therefore the value of the minimum cut in $G'$ is a constant factor approximation to the value of the minimum cut in $G$.
  \end{proof}
  
  \noindent Lastly, observe that this transformation can easily be performed in parallel by using a work-efficient connected components algorithm to perform the edge contractions, as is standard (see e.g.~\cite{karger1996new}).
  
  \subsection{Sampling the skeleton from a weighted graph} Note that by definition, the $p$-skeleton of a graph has $O(pm)$ edges in expectation. For a weighted graph, the $p$-skeleton is defined as the $p$-skeleton of the corresponding unweighted multigraph in which an edge of weight $w$ is replaced by $w$ parallel multiedges. The $p$-skeleton of a weighted graph therefore has $O(pW)$ edges in expectation, where $W$ is the total weight in the graph. Karger gives an algorithm for generating a $p$-skeleton in $O(pW \log(m))$ work, which relies on performing $O(pW)$ independent random samples with probabilities proportional to the weight of each edge, each of which takes $O(\log(m))$ amortized time. In Karger's algorithm, given a guess of
  the minimum cut $c$, he computes $p$-skeletons for $p = \Theta(\log(n)/c)$, which results in a skeleton of $O(m \log(n))$ edges, and hence takes $O(m \log^2(n))$ work to compute.
  
  Our algorithm instead does the following. For each edge $e$ in the graph, sample a binomial random variable $x \sim B(w(e),p)$. The skeleton then contains the edge $e$ with weight $x$ (conceptually, $x$ unweighted copies of the multiedge $e$). This results in the same graph as if sampled using Karger's technique. In Appendix~\ref{sec:binomial}, we show how to use recent results on sampling binomial random variables to perform samples from $B(n',1/2)$ in $O(\log(n'))$ time w.h.p., and from $B(n',p)$ in $O(\log^2(n'))$ time w.h.p., for any $n' \leq N$ after $O(N^{1/2+\varepsilon})$ work preprocessing. Since we can preprocess the graph to have edge weights at most $O(m\log(n))$ (Lemma~\ref{lem:low-weight-transform}), this is no more than $O(m)$ work in preprocessing.
  
  At first glance, this does not improve on Karger's bounds, since we need to perform $O(\log^2(n))$ work per edge when sampling from $B(n,p)$. However, we use the fact that only the first sample of the graph needs to be this expensive. In Karger's algorithm, and by extension, our algorithm, subsequent samples always take $p$ as exactly half of the value of $p$ from last iteration, and hence we can use subsampling to only require random variables from $B(n,1/2)$. This means that we can perform up to $O(\log(n))$ rounds of subsampling in $O(m\log^2(n))$ total work, instead of $O(m\log^3(n))$ work.
  
  \subsection{Sparse certificates}
  A \emph{$k$-connectivity certificate} of a graph $G = (V,E)$ is a graph $G' = (V, E' \subset E)$ such that every cut in $G$ of weight at most $k$ has the same weight in $G'$. In other words, a $k$-connectivity certificate is a subgraph that preserves cuts of weight up to $k$. A $k$-connectivity certificate is called \emph{sparse} if it has $O(kn)$ edges.
  
  Cheriyan, Kao, and Thurimella~\cite{cheriyan1993scan} introduce a parallel graph search called \emph{scan-first search}, which they show can be used to generate $k$-connectivity certificates of undirected graphs. Here, we briefly note that the algorithm can easily be extended to handle weighted graphs. The scan-first search algorithm is implemented as follows
  
  \begin{algorithm}[H]
    \caption{Scan-first search~\cite{cheriyan1993scan}}
    \label{alg:scan_first_search}
    \small
    \begin{algorithmic}[1]
      \small
      \Procedure{SFS}{$G = (V,E)$ : \algtype{Graph}, $r$ : \algtype{Vertex}}
        \State Find a spanning tree $T'$ rooted at $r$
        \State Find a preorder numbering to the vertices in $T'$
        \State For each vertex $v \in T'$ with $v \neq r$, let $b(v)$ denote the neighbor of $v$ with the smallest preorder number
        \State Let $T$ be the tree formed by $\{v, b(v)\}$ for all $v \neq r$
      \EndProcedure
    \end{algorithmic}
  \end{algorithm}

  \noindent Using a linear work, low depth spanning tree algorithm, scan-first search can easily be implemented in $O(m)$ work and $O(\log(n))$ depth. Cheriyan, Kao, and Thurimella show that if $E_i$ are the edges in a scan-first search forest of the graph $G_{i-1} = (V, E \setminus (E_1 \cup ... E_{i-1}))$, then $E_1 \cup ... E_k$ is a sparse $k$-connectivity certificate. A sparse $k$-connectivity certificate can therefore be found in $O(km)$ work and $O(k \log(n))$ depth by running scan-first search $k$ times.
  
  In the weighted setting, we treat an edge of weight $w$ as $w$ parallel unweighted multiedges. As always, this is only conceptual, the multigraph is never actually generated. To compute certificates in weighted graphs, we therefore use the following simple modification. After computing each scan-first search tree, instead of removing the edges present from $G$, simply lower their weight by one, and remove them only if their weight becomes zero. It is easy to see that this is equivalent to running the ordinary algorithm on the unweighted multigraph. We therefore have the following.
  
  \begin{lemma}
    Given a weighted, undirected graph $G = (V,E)$, a sparse $k$-connectivity certificate can be found in $O(km)$ work and $O(k \log(n))$ depth.
  \end{lemma}
  
  \subsection{Parallel Matula's algorithm for weighted graphs}
  Matula~\cite{matula1993linear} gave a linear time sequential algorithm for a $(2+\varepsilon)$-approximation to edge connectivity (unweighted minimum cut). It is easy to extend to weighted graphs so that it runs in $O(m \log(n) \log(W))$ time, where $W$ is the total weight of the graph. Using standard transformations to obtain polynomially bounded edge weights, this gives an $O(m \log^2(n))$ algorithm. Karger and Motwani~\cite{karger1994derandomization} gave a parallel version of Matula's unweighted algorithm that runs in ${O}(m^2/n)$ work. We will show that a slight modification to this algorithm makes it work on weighted graphs in $O(dm \log(W/m))$ work and $O(d \log(n) \log(W))$ depth, where $d$ is the minimum weighted degree of the graph. When $d = O(\log(n))$ and $W = O(m \polylog(n))$, this results in a final work bound of $O(m \log(n) \log\log(n))$.
  
  Essentially, Karger and Motwani's version of Matula's algorithm does the following steps as indicated in Algorithm~\ref{alg:matula}.
  
  \begin{algorithm}[H]
    \caption{Approximate minimum cut}
    \label{alg:matula}
    \small
    \begin{algorithmic}[1]
      \small
      \Procedure{Matula}{$G = (V,E)$ : \algtype{Graph} }
        \State \alglocal{} $d$ \algassign{} minimum degree in $G$
        \State \alglocal{} $k$ \algassign{} $d / (2 + \varepsilon)$
        \State \alglocal{} $C$ \algassign{} Compute a sparse $k$-certificate of $G$
        \State \alglocal{} $G'$ \algassign{} Contract all non-certificate edges of $E$
        \State \algreturn{} $\min(d, \textproc{Matula}(G'))$
      \EndProcedure
    \end{algorithmic}
  \end{algorithm}
  
  It can be shown that at each iteration, the size of the graph is reduced by a constant factor, and hence there are at most $O(\log(n))$ iterations. Furthermore, the work performed at each step is geometrically decreasing, so the total work, using the sparse certificate algorithm of Cheriyan, Kao, and Thurimella~\cite{cheriyan1993scan} is $O(dm)$ and the depth is $O(d \log^2(n))$.
  
  To extend the algorithm to weighted graphs, we can replace the sparse certificate routine with our modified version for weighted graphs, and replace the computation of $d$ with the equivalent weighted degree. By interpreting an edge-weighted graph as a multigraph where each edge of weight $w$ corresponds to $w$ parallel multiedges, we can see that the algorithm is equivalent. To argue the cost bounds, note that like in the original algorithm where the size of the graph decreases by a constant factor each iteration, the total weight of the graph must decrease by a constant factor in each iteration. Because of this, it is no longer true that the work of each iteration is geometrically decreasing. Naively, this gives a work bound of $O(d m \log(W))$, but we can tighten this slightly as follows. Observe that after performing $\log(W/m)$ iterations, the total weight of the graph will have been reduced to $O(m)$, and hence, like in the sequential algorithm, the work must subsequently begin to decrease geometrically. Hence the total work can actually be bounded by $O(d m \log(W/m) + dm) = O(dm \log(W/m))$. We therefore have the following.
  
  \begin{lemma}\label{lem:parallel-matula}
    Given an undirected, weighted graph $G$ with minimum weighted-degree $d$ and total weight $W$, a constant-factor approximation to the minimum cut can be computed in $O(dm\log(W/m))$ work and $O(d \log(n) \log(W))$ depth.
  \end{lemma}
  
  
  \subsection{A parallel approximation algorithm for minimum cut}

  The final ingredient needed to produce the parallel minimum cut approximation is a trick due to Karger. Recall that to produce Karger's skeleton graph, the sampling probability must be inversely proportional to the weight of the minimum cut, which paradoxically is what we are trying to compute. This issue is solve by using \emph{doubling}. The algorithm makes successively larger guesses of the minimum cut and computes the resulting approximation. It can then verify whether the guess was too high by checking whether the minimum cut in the skeleton contained too few edges (Lemma~\ref{lemma:sampling_verified}). Specifically, Karger's sampling theorem~(Lemma 6.3.2 of \cite{karger1995random}) says that we will know that we have made the correct guess within a factor two when the skeleton has $\Omega(\log(n))$ edges in its minimum cut. To perform the minimum amount of work, we use Lemma~\ref{lem:k-approx} to first produce a $O(\log(n))$-approximation to the minimum cut, which allows us to make just $O(\log\log(n))$ guesses with the guarantee that one of them will be correct to within a factor two.
  
  Our algorithm proceeds by making these $O(\log\log(n))$ guesses in parallel. For each, we consider the corresponding skeleton graph and compute a $\Theta(\log(n))$ certificate, since, by assumption, until we have made the correct guess, the minimum cut in the skeleton will be less than $O(\log(n))$ w.h.p. This then guarantees that we can run our version of parallel Matula's algorithm in $O(n \log(n) \log\log(n))$ work (Lemma~\ref{lem:parallel-matula}), since, after producing the certificate, the total weight of the graph is at most $O(n \log(n))$, and the minimum degree is no more than $O(\log(n))$. The details are depicted in Algorithm~\ref{alg:approx_min_cut}. It takes $O(m\log^2(n))$ work to produce the sequence of graph skeletons, $O(m\log(n)\log\log(n))$ work to compute the sparse certificates, and $O(n\log(n)(\log\log(n))^2)$ work to compute the resulting approximations from Matula's algorithm. All together, the algorithm takes at most $O(m\log^2(n))$ work, and runs in $O(\log^3(n))$ depth.
  
  \begin{algorithm}
    \caption{Approximate minimum cut algorithm}
    \label{alg:approx_min_cut}
    \small
    \begin{algorithmic}[1]
      \small
      \Procedure{ApproxMinCut}{$G = (V,E)$ : \algtype{Graph} }
        \State\label{code:logn-approx} \alglocal{} $C$ \algassign{} A $\log(n)$-approximation of MinCut($G$)
        \ParallelFor{$c \in \{ C/\log(n), 2C/\log(n), ... C \}$}
          \State $p(c)$ \algassign{} $\Theta(\log(n)/c)$
          \State \alglocal{} $G_p$ \algassign{} Compute the skeleton graph $G'(p)$
          \State \alglocal{} $G_p'$ \algassign{} Compute a $\Theta(\log(n))$-certificate of $G_p$
          \State $\hat{c}(c)$ \algassign{} \textproc{Matula}($G_p'$)
        \EndParallelFor

        \If{$\hat{c}(C/\log(n)) \leq O(\log(n))$}
          \State \algreturn{} $\hat{c}(C/\log(n))$
        \Else
          \State \alglocal{} $c$ \algassign{} $\min \{ c\ |\ \hat{c}(c) \geq O(\log(n)) \}$
          \State \algreturn{} $\hat{c}(c) / p(c)$
        \EndIf
      \EndProcedure
    \end{algorithmic}
  \end{algorithm}
  
  \noindent To see that the final returned value is correct, we appeal to Karger's sampling theorem, which says that w.h.p., if our guess of the minimum cut is too high by a factor two, the minimum cut of the skeleton will have less than $O(\log(n))$ edges w.h.p.~\cite{karger1995random}, and hence the certificate algorithm does not damage the minimum cut. Once our guess is below the minimum cut by a factor two, the sampling theorem says that the minimum cut of the skeleton exceeds $\Omega(\log(n))$. Provided that we set the constant of the $\Theta(\log(n))$ certificate to be a constant factor larger than this threshold, a Chernoff bound shows us that one of our guesses leads to a skeleton with approximate minimum cut $\hat{c} = \Omega(\log(n))$ that is not damaged by the certificate, and then Lemma~\ref{lemma:sampling_verified} says that $\hat{c} / p$ is a constant-factor approximation of the minimum cut w.h.p.
  This argument works only if the minimum cut of $G$ has size at least $\Omega(\log(n))$, but note that if it does not, the skeleton construction $G'(1)$ (which must occur during the last iteration) and the certificate completely preserve the minimum cut and hence the last iteration of the loop finds a constant factor approximation of the minimum cut in $G$.
  
  \begin{comment}
  \paragraph{An error in Karger's algorithm} In \cite{karger2000minimum}, Corollary 4.2, Karger claims that he can produce the set of $O(\log(n))$ spanning trees with $O(m + n \log(n))$ processors in $O(\log^3(n))$ time (equivalent to $O(m\log^3(n) + n\log^4(n))$ work and $O(\log^3(n))$ depth in our model). In his proof, he claims that the skeleton construction can be performed the same as in the sequential case and is trivial to parallelize. He cites ``[Karger 1994a]'', which is missing from the bibliography, but it likely meant to refer to his PhD thesis~\cite{karger1995random}. However, we note that there is at least one non-trivial difference between the sequential and parallel sampling algorithms, which is the approximate minimum cut that is used to compute the sampling probability. The sequential algorithm uses Matula's algorithm~\cite{matula1993linear} to obtain this approximation. In his thesis~\cite{karger1995random} and in the paper~\cite{karger1994using}, Karger gives a parallelization of Matula's algorithm for unweighted graphs that he claims runs in $O(cm \polylog(n))$ work (Theorem 4.1 of \cite{karger1994using} or Lemma 5.2.8 of \cite{karger1995random}), where $c$ is the size of the minimum cut. However, we note that the work of the algorithm is dependent on the computation of an $O(d)$-certificate, where $d$ is the minimum degree of the graph, a subroutine that takes $\Omega(dm)$ work using either the sparse certificate algorithm of Cheriyan, Kao, and Thurimella~ \cite{cheriyan1993scan}, or Karger's own sparse certificate algorithm~\cite{karger1994derandomization}. The runtime should therefore be proportional to $d$. In the reduction to solve the weighted case, Karger takes a skeleton of the weighted graph, which has minimum cut $O(\log(n))$, but is not guaranteed to have low degree. His remark following Theorem 4.1 of \cite{karger1994using} that the skeleton ought to have $O(n \polylog(n))$ edges suggests that he also intended to take a sparse $O(\log(n))$ certificate of the skeleton, which would result in the skeleton having low degree, though this is not stated. In a later work with Karger and Motwani~\cite{karger1994derandomization}, they give a correct bound of $O(m^2/n)$ for the unweighted algorithm. We therefore believe that Karger's bounds as stated in Corollary 4.2 of \cite{karger2000minimum} are not justified. Our result (Theorem~\ref{thm:tree-packing}) corrects this.
  \end{comment}
  

==> batch-add-path.tex <==
\section{Bulk Path Updates For RC Trees}\label{sec:batch-addpath}

Given an RC tree of a tree on $n$ vertices and a set of $k$ path updates of the form $(v_i, x_i)$, denoting that $x_i$ is to be added to the weight of all edges on the path from $r$ to $v_i$, we can apply all of them in $O(n)$ work and $O(\log(n))$ depth w.h.p. The idea is similar to a standard treefix sum algorithm. First, the algorithm associates each vertex $v_i$ with its weight $x_i$. Now the operation is to add to each edge $(u,v)$, where $v$ is a child of $u$, the weight of all vertices in the subtree rooted at $v$. The algorithm then proceeds in two steps. First, in a traversal of the RC tree, it computes, for each cluster $C$, the total weight $W(C)$ of all vertices in it. This step is the same as the first step of our batched mixed operations algorithm, and takes $O(n)$ work and $O(\log(n))$ depth w.h.p.
Second, for each child cluster of the root, it traverses the RC tree top-down, maintaining the weight $w$ of all vertices that are descendants of the current cluster (initially zero). This is achieved when recursing on $\ra{C}{t}$, by adding $W(C) - W(\ra{C}{t})$ to the accumulated weight $w$, otherwise keeping $w$ the same. When reaching a base edge cluster, the value $w$ is added to the weight of the edge. This takes $O(n)$ work and $O(\log(n))$ depth w.h.p.


==> batch-component-weight.tex <==
\section{Mixed Component Weight Operations}\label{sec:batch-component-weight}

Here, we describe a simple RC implementation of the following operations, which is hence amenable to our batched mixed operations framework.
\begin{itemize}[leftmargin=*]
  \setlength\itemsep{0em}
  \item \textproc{SubtractWeight}($v, w$): Subtract weight $w$ from vertex $v$
  \item \textproc{JoinEdge}($e$): Mark the edge $e$ as ``joined''
  \item \textproc{QueryWeight}($v$): Return the weight of the connected component containing the vertex $v$, where the components are induced by the joined edges 
\end{itemize}

\noindent The values stored in the RC clusters are as follows. Vertices store their weight, and unary clusters store the weight of the component reachable via joined edges from the boundary vertex. A binary cluster is either \emph{joined}, meaning that its boundary vertices are connected by joined edges, in which case it stores a single value, the weight of the component reachable via joined edges from the boundaries, otherwise it is \emph{split}, in which case it stores a pair: the weight of the component reachable via joined edges from the top boundary, and the weight of the component reachable via joined edges from the bottom boundary. We provide pseudocode for the update operations for Illustration in Algorithm~\ref{alg:component-weight}.

\begin{algorithm}
    \begin{algorithmic}[1]
      \small
      \Procedure{$f_{\mbox{\small unary}}$}{$v_v, t, U$}
        \If{t = $(t_v, b_v)$}
          \algreturn{} $t_v$
        \Else\ 
          \algreturn{} $v_v + t + \sum_{u_v \in U} u_v$
        \EndIf
      \EndProcedure 
      \Procedure{$f_{\mbox{\small binary}}$}{$v_v, t, b, U$}
        \If{$t = t_v$ and $b = b_v$}
          \State \algreturn{} $t_v + b_v + v_v + \sum_{u_v \in U} u_v$
        \ElsIf{$t = (t_{t_v}, t_{b_v})$ \algand{} $b = b_v$}
          \State \algreturn{} $(t_{t_v}, t_{b_v} + v_v + b_v + \sum_{u_v \in U} u_v)$
        \ElsIf{$t = t_v$ \algand{} $b = (b_{t_v}, b_{b_v})$}
          \State \algreturn{} $(t_v + v_v + b_{t_v} + \sum_{u_v \in U} u_v)$
        \ElsIf{$t = (t_{t_v}, t_{b_v})$ \algand{} $b = (b_{t_v}, b_{b_v})$}
          \State \algreturn{} $(t_{t_v}, b_{b_v})$
        \EndIf
      \EndProcedure
\Procedure{SubtractWeight}{$v, w$}
   \State $\ra{v}{\text{value}}$ \algassign{} $\ra{v}{\text{value}}$ - $w$
   \State Reevaluate the $f(\cdot)$ on path to root.
\EndProcedure
\Procedure{JoinEdge}{$e$}
  \State $\ra{e}{\text{value}}$ \algassign{} 0
  \State Reevaluate the $f(\cdot)$ on path to root.
\EndProcedure
    \end{algorithmic}
    \caption{A \simpleRC{} implementation of \textproc{SubtractWeight} and \textproc{JoinEdge}.}
    \label{alg:component-weight}
\end{algorithm}

\noindent The initial value of a vertex is its starting weight. The initial value of an edge is $(0, 0)$, indicating that it is split at the beginning. Note that $f_{\mbox{\small unary}}$ and $f_{\mbox{\small binary}}$ can be evaluated in constant time, and the structure of the updates involves setting the value at a leaf using an associative operation and re-evaluating the values of the ancestor clusters.

We can argue that the values are correctly maintained by structural induction. First consider unary clusters. If the top subcluster is split, then the representative vertex and unary subclusters are not reachable via joined edges, and hence the only reachable component is the component reachable inside the top subcluster from its top boundary, whose weight is $t_v$. If the top subcluster is joined, then the representative vertex is reachable, which is by definition the boundary vertex of the unary subclusters, and hence the reachable component is the union of the reachable components of all of the subclusters, whose weight is as given. 

For binary clusters, there are four possible cases, depending on whether the top and bottom subclusters are joined or not. If both are joined, then the representative and hence the boundary of all subclusters is reachable from both boundaries, and hence the cluster is joined and the reachable component is the union of the reachable components of the subclusters. If either subcluster is split, then the reachable component at the corresponding boundary is just the reachable component of the subcluster, whose weight is as given. Lastly, if one of the subclusters is not split, then the corresponding boundary can reach the representative vertex, and hence the reachable components of the unary subclusters, whose weights are as given.

It remains to argue that we can implement \textproc{QueryWeight} with a simple RC implementation. Consider a vertex $v$ whose component weight is desired and consider the parent cluster $P$ of $v$, i.e.,\ the cluster of which $v$ is the representative. If $P$ has no binary subclusters that are joined, observe that $P$ must contain the entire component of $v$ induced by joined edges, since the only way for a component to exit a cluster is via a boundary which would have to be joined. Answering the query in this situation is therefore easy; the result is the sum of the weights of $v$, the unary subclusters of $P$, the bottom boundary weight of the top subcluster (if it exists), and the top bounary weight of the bottom subcluster (if it exists). Suppose instead that $P$ contains a binary subcluster that is joined to some boundary vertex $u \neq v$. Since the subcluster is joined, $u$ is in the same induced component as $v$, and hence \textproc{QueryWeight}($v$) has the same answer as \textproc{QueryWeight}($u$). By standard properties of RC trees, since $u$ is a boundary of $P$, we also know that the leaf cluster $u$ is the child of some ancestor of $P$. Since the root cluster has no binary subclusters, this process of jumping to joined boundaries must eventually discover a vertex that falls into the easy case, and since such a vertex $u$ is always the child of some ancestor is $P$, the algorithm only examines clusters that are on or are children of the root-to-$v$ path in the RC tree, and hence the algorithm is a simple RC implementation.


==> dynamic-tree-implementation.tex <==
\section{Dynamic tree data structures}\label{sec:dynamic-trees}
  
  
  
  \begin{comment}
  \paragraph{Deterministic vs randomized RC trees}
  
  RC trees have previously been implemented using randomized tree contraction algorithms~\cite{acar2005experimental,acar2020batch}. The primary reason for this is because the randomized algorithms can be shown to be \emph{dynamizable}~\cite{acar2004dynamizing}, that is, it is possible to perform structural changes to the tree, such as inserting or deleting edges, and to update the resulting tree contraction efficiently without running it from scratch. It is not known how to do this using the deterministic variants of tree contraction. However, since our algorithms only make \emph{value updates} to the tree, e.g., changing edge weights, and do not make structural changes, we can implement RC trees using the deterministic tree contraction algorithm of Gazit, Miller, and Tate~\cite{gazit1988optimal}. This means that the randomized bounds usually obtained by the use of RC trees can be made deterministic.
  \end{comment}
  
  \begin{comment}
  \subsection{Parallel batch-dynamic subtree queries with path updates}\label{sec:batchtrees}
  
  We now present the batch-dynamic algorithm that can perform $k$ queries and updates
  in $O(k\log(1+n/k))$ work and $O(\log(n))$ depth. 
  As in the
  non-batched case, the algorithm first computes a static RC tree of the rooted tree
  $T$, which takes $O(n)$ work and $O(\log(n))$ depth. Each cluster node stores the same augmented values as in the non-batch case.
  
  \paragraph{Updates} A naive batch update algorithm would first generate all of the clusters in the path decompositions of all the paths. This would take $O(k \log(n))$ work, though, which already exceeds our desired time bounds. The trick to obtain improved bounds is to work incrementally from the bottom of the RC tree and combine updates on the way up. We assume that the batch of updates contains no duplicate vertices. This is easily achieved by preprocessing the batch and combining duplicates if there are any.
  
  We use the fact that given a cluster in the RC tree, we can easily determine the next cluster above it in a path decomposition in constant time (Lemma~\ref{lem:path_decomposition}). The algorithm determines, for each update, the first cluster on the path decomposition, and then processes the clusters level by level. At the lowest level of each update, the cluster $C$ is annotated with a value $p_{\text{update}}(C)$, containing the amount $x$ that will be added to that cluster.
  The algorithm then works level-by-level bottom up, for each affected cluster $C$, adds $p_{\text{update}}(C)$ to $p_+(C)$ and then recomputes the values of $p_{\min}$ and $w_{\min}$ using their recurrence relations. If $C$ has a subsequent cluster $C'$ in the path decomposition, then $C'$ is added to the list of affected clusters, and $p_{\text{update}}(C')$ is incremented by $p_{\text{update}}(C)$. The same $C'$ may be incremented concurrently by multiple predecessors, but since it can only have a constant number of predecessors per level, this is easy to implement in constant time.
  
  Since we only perform constant work for each node in the RC tree that is an ancestor of one of the update leaves, Lemma~\ref{lem:batch-bound} implies that the work of the algorithm is $O(k \log(1+n/k))$. Since the algorithms processes level-by-level and takes constant time per level and the RC tree has $O(\log(n))$ height, the update algorithm has $O(\log(n))$ depth.

  \begin{algorithm}[h]
    \caption{Batch path update algorithm}
    \label{alg:batch_path_update}
    \begin{algorithmic}[1]
      \Procedure{BatchAddPath}{$U = \{ (v_i, x_i) \}$ : \algtype{(vertex, number) list } }
      \State \alglocal{} N \algassign{} \textproc{Ancestors}($\{ \{ v_i \} \}$) $\cup$ \textproc{Children}(\textproc{Ancestors}($\{ \{ v_i \} \}$))
      \State \alglocal{} $p_{\text{update}}(C)$ \algassign{} $0$ for each $C \in N$
      \ParallelFor{\algeach{} $(v, x) \in U$}
      \State \alglocal{} $C$ \algassign{} $\textproc{FirstClusterInPathDecomposition}(v)$
      \State $p_{\text{update}}(C)$ \algassign $x$
      \EndParallelFor
      \ParallelFor{\algeach{} level of nodes $N_i \in N$, bottom up}
      \ParallelFor{\algeach{} cluster node $C \in N_i$}
      \State $p_+(C)$ \algassign{} $p_+(C) + p_{\text{update}}(C)$
      \State \textproc{UpdateCluster}($C$)
      \If{$p_{\text{update}}(C) \neq 0$ \algand{} $\textproc{TopBoundary}(C) \neq r$}
      \State \alglocal{} $P$ \algassign{} \textproc{NextClusterInPathDecomposition}($C$)
      \State \textproc{FetchAndAdd}($p_{\text{update}}(P), p_{\text{update}}(C)$)
      \EndIf
      \EndParallelFor
      \EndParallelFor
      \EndProcedure
    \end{algorithmic}
  \end{algorithm}

  
  \paragraph{Subtree queries} Subtree queries use some similar ideas from the sequential case, and some new ones. First, as is the same in the sequential case, the algorithm must aggregate the sums of the $p_+$ values for contiguous paths of binary clusters. This can be performed in exactly the same way, but traversing the tree in parallel.
  
  To parallelize computing the lightest edge in multiple subtrees requires an additional pair of observations. First, the subtree decomposition for a vertex $v$ consists of constant number of clusters plus the subtree decomposition of at most one other vertex. Secondly, the other subtree decomposition on which the first one depends always corresponds to a vertex higher in the RC tree. This means that we can traverse the RC tree top down and fill in the values of the subtree queries. Each query is the minimum of a constant number of unary cluster minimums, and at most one other subtree minimum, which will have already been computed since it is at a higher level. 
  
  \begin{algorithm}[H]
    \caption{Batch subtree query algorithm}
    \label{alg:batch_subtree_query}
    \begin{algorithmic}[1]
      \Procedure{BatchQuerySubtree}{$Q = \{ v_i \}$ : \algtype{vertex list } }
      \State \alglocal{} N \algassign{} \textproc{Ancestors}($\{ \{ v_i \} \}$) $\cup$ \textproc{Children}(\textproc{Ancestors}($\{ \{ v_i \} \}$))
      \State \alglocal{} $p_\text{extra}(C)$ \algassign{} $0$ for each $C \in N$
      \For{\algeach{} cluster node $C$ in a parallel top-down traversal of $\textproc{Ancestors}(Q)$}
      \If{$C$ \algis{} a \algtype{binary cluster}}
      \For{\algeach{} \algtype{binary cluster} $B$ \algin{} \textproc{BinaryChildren}($C$)}
      \State $p_{\text{extra}}(B)$ \algassign{} $p_{\text{extra}}(C)$ + $p_+(C)$
      \EndFor
      \EndIf
      \EndFor
      \State \alglocal{} answer($v$) \algassign{} $\infty$ for each $v \in Q$
      \For{\algeach{} cluster node $C$ in a parallel top-down traversal of $N$}
      	\If{$C = \{ v \}$ for some $v \in Q$}
      		\State answer($v$) = $\min_{c \in \textproc{UnaryChildren}(\textproc{Cluster}(v))} w_{\min}(c)$
          \If{\textproc{Cluster}($v$) \algis{} a \algtype{binary cluster}}
            \State \alglocal{} bottom\_edge \algassign{} \textproc{Bottom}(\textproc{Cluster}($v$))
            \State \alglocal{} edge\_weight \algassign{} $\min(w_{\min}(\text{bottom\_edge}), p_{\min}(\text{bottom\_edge}) + p_{\text{extra}}(\text{bottom\_edge}))$
            \State answer($v$) \algassign{} $\min(\text{answer}(v), \text{edge\_weight})$
            \State answer($v$) \algassign{} $\min(\text{answer}(v), \text{answer}(\textproc{BottomBoundary}(\text{bottom\_edge})))$ 
          \EndIf
      	\EndIf
      \EndFor
      \EndProcedure
    \end{algorithmic}
  \end{algorithm}
  
  \paragraph{Edge queries} Edge queries are very similar. The contiguous sums of $p_+$ are aggregated down the tree, and the resulting values are read off the binary clusters corresponding to the edges.
  
  \begin{algorithm}[H]
  	\caption{Batch edge query algorithm}
  	\label{alg:batch_edge_query}
  	\begin{algorithmic}[1]
  		\Procedure{BatchQueryEdge}{$Q = \{ e_i \}$ : \algtype{vertex list } }
  		\State \alglocal{} $p_\text{extra}(C)$ \algassign{} $0$ for each $C \in \textproc{Ancestors}(Q)$
  		\ParallelFor{\algeach{} level of nodes $N_i \in \textproc{Ancestors}(Q)$, top down}
  		\ParallelFor{\algeach{} cluster node $C \in N_i$}
  		\If{$C$ \algis{} a \algtype{binary cluster}}
  		\For{\algeach{} \algtype{binary cluster} $B$ \algin{} \textproc{BinaryChildren}($C$)}
  		\State $p_{\text{extra}}(B)$ \algassign{} $p_{\text{extra}}(C)$ + $p_+(C)$
  		\EndFor
  		\EndIf
  		\EndParallelFor
  		\EndParallelFor
  		\State \alglocal{} answer($e$) \algassign{} ($p_{\min}(\{e\}) + p_{\text{extra}}(\{ e \})$) for each $e \in Q$
  		\State \algreturn{} answer
  		\EndProcedure
  	\end{algorithmic}
  \end{algorithm}
  \end{comment}
  
  
  
  

==> dynamic-trees.tex <==
 \section{Batched mixed operations on trees }\label{sec:tree-ops}
    The key part of Geissmann and Gianinazzi's parallel minimum cut algorithm~\cite{geissmann2018parallel} is a data structure that can evaluate a sequence of path weight updates and path weight queries on a tree all in parallel as if the operations were executed sequentially. This allows their algorithm to simulate the steps of Karger's sequential algorithm in low depth. In this section, we introduce a framework that both generalizes and improves on the work bounds of this data structure. Our framework can take any suitable set of weighted tree update and query operations and produce an algorithm for simulating them work efficiently in low depth. This framework is based on parallel RC trees.
    
    \begin{definition}[Simple Operations]
      We say that a sequence of update and query operations on a rooted RC tree is \emph{simple} if
      \begin{itemize}[leftmargin=*]
          \item An augmented value is maintained at every cluster that is set directly at the leaves, and can be computed for internal clusters in constant time given the values of the children clusters
          \item Update operations involve modifying an augmented value at a leaf and then propagating the updated augmented values to each ancestor cluster as above
          \item Query operations need only examine the values on clusters on a root-to-leaf path and their children
      \end{itemize}
    \end{definition}
    
    \noindent Properties~\ref{lem:path_decomposition}~and~\ref{lem:subtree-decomposition} suggest that path and subtree operations are simple and therefore amenable to this framework. We will show that they can be implemented as such.
    
    \begin{theorem}
      Given a sequence of $k$ simple operations on a rooted RC tree, there exists an algorithm that can compute the result of all of the query operations as if the sequence of updates and queries was executed sequentially, in $O(n + k\log(n+k))$ work and $O(\log(n)\log(k))$ depth.
    \end{theorem}
    
    \subsection{Batch evaluation algorithm}\label{sec:batcheval}
      
       As in the non-batched case, the algorithm first computes a static RC tree of the rooted tree $T$, and computes the initial values of the augmented data ($p_{\min}$ and $w_{\min}$) which takes $O(n)$ work and $O(\log(n))$ depth. We use similar techniques to Geissmann and Gianinazzi~\cite{geissmann2018parallel},
      in which we merge sorted update sequences up the tree so that each
      node of the RC tree knows its value at all relevant times.  \guy{the
        previous sentence makes our result sound incremental.   we should
        point out issues with previous approach.}
    At a high
      level, the algorithm works in three phases. In the first phase, the
      algorithm delivers all of the direct updates (i.e.\ $p_+$ values)
      \guy{perhaps not clear what direct updates are.}  to the relevant nodes. In the second phase, the algorithm traverses the RC tree bottom-up, for each node, merging the updates (based on their order in the operation sequence) present in its children. At the end of these two phases, every node knows its relevant values at all times at which it was affected by an update. Finally, queries can now be performed by looking up the values in the nodes that they depend on after the most recent update. We now describe these ideas in more detail.
      
      For each operation in the operation sequence, we first tag it with a
      timestamp $t$, given by its position in the sequence. This allows us
      to correctly order sequences of updates that affect the same values,
      and answer queries with respect to only the previous updates. For
      each node, instead of storing a single value of $p_{\min}$, $w_{\min}$, and $p_+$, the algorithm stores a timestamped list of values. Let's use the following notation to make things clearer
      \begin{itemize}
        \item $p^t_{\min}(B)$ denotes the minimum weight on the cluster path of $B$ at timestamp $t$.
        \item $w^t_{\min}(C)$ denotes the minimum weight in the cluster $C$ at timestampt $t$
        \item $p^t_+(B)$ denotes the amount of weight directly added to cluster $B$ during timestamp $t$
        \item $p^t_{\Sigma}(B)$ denotes the sum of all weights added directly to cluster $B$ up to and including timestamp $t$.
      \end{itemize}
      Assume that the initial values (before applying any updates)
      correspond to timestamp $0$, and the first operation starts from
      timestamp $1$. For a cluster $C$, we denote the list of
      \emph{relevant timestamps} by $\mathbf{t}(C)$. A timestamp is
      relevant to a node if its value could change at that timestamp due
      to an update that occurred at that time. \guy{wordy.}
      
      \paragraph{Phase one: Delivering updates to nodes.}
      
      The goal of phase one is for each binary cluster in the path
      decomposition of any of the updates to have a list of timestamped
      update operations that affected it. In other words, the goal is to
      populate $p_+(B)$ for all affected binary clusters. Naively, we
      could achieve this by generating the path decomposition for every
      update, bucketing the update operations into the clusters, and
      sorting them. However, since there are $O(k \log(n))$ total clusters
      in all of the path decompositions w.h.p., sorting them all would take $O(k
      \log(n) \log(k))$ work, which is a $\log(k)$ factor too
      high. In the sequential setting, a stable radix sort could be used instead, but there is no known parallel stable radix sort algorithm that runs in low depth. We therefore use a more clever approach.
      
      Recall that for simplicity, all path updates are on paths of the form $r-v$, where $r$ is the root
      vertex of the tree. The algorithm begins by bucketing the update
      operations based on the vertex $v$ and sorting them in order of
      their timestamp within each bucket. This can be achieved with a parallel sorting
      algorithm and hence takes $O(k\log(k))$ work and $O(\log(k))$
      depth w.h.p. We now take advantage of the fact that the clusters in the
      path decomposition of any $v-r$ path are all children of
      clusters on the $v$ to root path in the RC tree. The main idea is
      then to walk up the tree in parallel from each affected $v$ in level
      order, merge \guy{by timestamp?} the updates that were present on the children clusters, and then deliver any updates that need to be delivered to one of the children. Observe that in total, each update operation touches $O(\log(n))$ nodes in the RC tree w.h.p, for a total of $O(k \log(n))$ updates w.h.p. At each node, the algorithm can use a work-efficient merge routine which preserves the timestamp order of the updates and runs in linear work and $O(\log(k))$ depth. Therefore phase one takes $O(k \log(n) + k\log(k))$ total work w.h.p., which is at most $O(k \log(n+k))$ w.h.p. Since there are $O(\log(n))$ levels in the RC tree w.h.p.\ and each one can be processed in parallel, it takes $O(\log(n)\log(k))$ depth w.h.p.
      
      \paragraph{Phase two: Merging updates.}
      
      After phase one, every binary cluster will contain the relevant
      updates \guy{what are relevant updates?} in its $p_+$ list. Phase two is to apply the result of these updates to the augmented data $p_{\min}$ and $w_{\min}$ and recursively update the ancestors augmented data. Recall from earlier that in the non-timestamped case, the augmented values were computed in terms of the augmented values of the child clusters. We use a similar idea in the timestamped case, except that we must now merge the relevant timestamp lists of the children, and then compute the augmented value at each timestamp, which will depend on the augmented values of the children at the most recent timestamp.
      
      First, set the relevant timestamps of each cluster to $\{0\}$. The relevant timestamps for each cluster are then the union of those of their children, and the timestamps at which the cluster was updated, i.e.\ those at which $p^t_+(C) \in p_+(C)$. For a binary cluster, we can use a parallel prefix sum (scan) algorithm to compute $p^t_{\Sigma}(B)$ for every relevant timestamp $t \in \mathbf{t}(B)$, since, by definition
      \begin{equation}
      p^t_{\Sigma}(B) = \sum_{\substack{t' \in \mathbf{t}(B), t' \leq t}} p^{t'}_+(B).
    \end{equation}
      This takes linear work in the number of relevant timestamps and $O(\log(k))$ depth. Then, we can calculate the timestamped values using the following recurrences. For binary clusters $B$ with subclusters $c(B)$ and binary subclusters $B^\uparrow$ and $B^\downarrow$
      \begin{itemize}
        \item $p^t_{\min}(B) = \min(p^{t'}_{\min}(B^\uparrow), p^{t''}_{\min}(B^\downarrow)) + p^t_\Sigma(B)$, where $t' = \max \{ \mathbf{t}(B^\uparrow) \leq t \}$, $t'' = \max \{ \mathbf{t}(B^\downarrow) \leq t \}$
        \item $w^t_{\min}(B) = \min( p^t_{\min}(B), \displaystyle\min_{c \in c(B)} w^{t_{c}}_{\min}(c) )$ where $t_{c} = \max \{ \mathbf{t}(c) \leq t \}$
      \end{itemize}
      For non-binary clusters $C$ with subclusters $c(C)$,
      \begin{itemize}
        \item $w^t_{\min}(C) =\displaystyle\min_{c \in c(C)} w^{t_{c}}_{\min}(c)$ where $t_{c} = \max \{ \mathbf{t}(c) \leq t \}$
      \end{itemize}
      Naively, we could compute the values of $t', t''$ and $t_{c_i}$ using a binary search on the list of timestamps, but this would add an extra $\log$ factor to the work. To make this efficient, we can compute them all at once using a linear work merge on the children's timestamps. Each augmented value at each timestamp can then be computed in constant time. Since each update contributes a relevant timestamp to all of its ancestors, and their direct children, the total number of relevant timestamps across all nodes is $O(k \log(n))$ w.h.p. Since each node performs linear work in this quantity and takes $O(\log(k))$ depth, processing the $O(\log(n))$ levels of the tree in parallel, the total cost of phase two is $O(k \log(n))$ work and $O(\log(n)\log(k))$ depth w.h.p.
      
      
      \paragraph{Phase three: Answering queries.}
      
      The final phase is to answer all of the queries in the operation sequence. A naive algorithm for doing so would be to evaluate each query independently. Note that the sequential query algorithms inspect the values of at most $O(\log(n))$ clusters w.h.p.\ to determine their answers. This process can simply be performed independently in parallel for each query, using a binary search to determine the most recent $t' \in \mathbf{t}(C)$ for each cluster $C$ examined, to read the most up-to-date values of $p_{\min}$, $p_+$, and $w_{\min}$. Unfortunately, this algorithm incurs an extra $O(\log(k))$ work overhead due to the binary search. To mitigate this, we simply use the same trick as in phase one, where we bucket each query into the leaf cluster of the vertex/edge that it corresponds to, sort these buckets by timestamp, merge the buckets up the tree maintaining timestamp order, and copying queries to the children if they need to read them. Since, just like updates, queries only ever need to read values that are on or are children of the root-to-leaf path, this requires $O(k \log(n) + k\log(k))$ work in total w.h.p.\ and $O(\log(n)\log(k))$ depth using a linear work $O(\log(k))$ depth merge algorithm. Once the queries have been sorted and delivered, the binary searches can be replaced by merging the query list on each node with the list of relevant timestamps, just like in Phase Two, which also takes $O(k \log(n))$ work and $O(\log(k)\log(n))$ depth w.h.p. Finally, each query can now be answered in $O(\log(n))$ time w.h.p.\ by examining the relevant nodes and finding the correct timestamp to look at in $O(1)$ using the result of the merge. This phase therefore takes $O(k\log(n) + k\log(k))$ total work w.h.p., which is at most $O(k \log(n+k))$, and $O(\log(n)\log(k))$ depth w.h.p.
      
      
      
    
    \subsection{Dynamic subtree queries with path updates}\label{sec:seq-tree}
    
    We wish to maintain, given a rooted tree $T = (V,E)$ a weight
    $w(e)$ for each $e \in E$, a data structure that supports the following operations.
    \begin{itemize}[leftmargin=*]
      \item \textproc{AddPath}($u, v, x$): Adds $x$ to the weight of all edges on
      the path from $u \in V$ to $v \in V$,
      \item \textproc{QuerySubtree}($v$): Returns the smallest weight
        of an edge in the subtree rooted at $v \in V$,
      \item \textproc{QueryEdge}($e$): Returns $w(e)$
    \end{itemize}
\guy{do we need a QueryEdge?   Isn't it a 
  special case of QuerySubtree? Perhaps we have to add (inclusive) to
  the description of querysubtree.}

    \noindent This can be achieved in the sequential setting in $O(\log(n))$ time by using top trees~\cite{alstrup2005maintaining}. We will now show how to implement this using RC trees. Our solution matches the bounds of the canonical sequential solution given by top trees and link-cut trees; it solves a single query or performs a single update in $O(\log(n))$ time.
    
    To simplify the algorithms, we assume that path updates are only ever performed on root-to-vertex paths. This comes at no loss of generality since an update to an arbitrary path $u \to v$ can be performed in this setting by converting \textproc{AddPath}$(u,v,x)$ into \textproc{AddPath}$(r, v, x)$, \textproc{AddPath}$(r,u,x)$, \textproc{AddPath}$(r, \textproc{LCA}(u,v), -2x)$.
    
    Given as input, a rooted tree $T$ with root $r$, our algorithm builds a static
    RC tree~\cite{acar2005experimental,acar2020batch} on $T$. This can be achieved
    in $O(n)$ work and $O(\log(n))$ depth w.h.p.\ using
    the tree contraction algorithm of Miller and Reif~\cite{miller1985parallel}.
    Note that we do not need to employ fully dynamic RC trees since we only perform
    value updates to the tree, and never links or cuts.
    Nodes in the RC tree will be augmented to store the following
    information:

\guy{On rereading this I find the late introduction of lazyness
  confusing.   Perhaps we should say from the start something like` ``lazy minimum
  weight, where the actual min weight is calculated as described below''.}

    \begin{itemize}
      \item $w_{\min}(C)$: The minimum weight edge in the cluster $C$
        \guy{Technically it is the weigh of the minimum edge in the
          cluster, not the edge itself, right?}
    \end{itemize}
    \noindent Nodes corresponding to binary clusters will additionally store the following:
    \begin{itemize}
      \item $p_+(C)$: The total weight that has ever been directly added to the cluster path of $C$
      \item $p_{\min}(C)$: The minimum weight edge on the cluster path of $C$
    \end{itemize}
    
\guy{Are binary clusters denoted with $B$ or $C$.   We seem to be inconsistent.}
    \noindent $w_{\min}$ and $p_{\min}$ are initially computed and maintained using
    the following recurrence relations. Given a binary cluster $B$ with subclusters $c(B)$ and top and bottom binary subclusters
    $B^{\uparrow}$ and $B^{\downarrow}$, we have
    \begin{itemize}
      \item $p_{\min}(B) = \min(p_{\min}(B^{\uparrow}), p_{\min}(B^{\downarrow})) + p_+(B)$
      \item $w_{\min}(B) = \min(p_{\min}(B), \displaystyle\min_{c \in c(B)} w_{\min}(c))$
    \end{itemize}
    For a nonbinary cluster $C$ with subclusters $c(C)$, we similarly set
    \begin{itemize}
      \item $w_{\min}(C) = \displaystyle\min_{c \in c(C)} w_{\min}(c)$
    \end{itemize}
    
    \paragraph{Updates.}
    To implement \textproc{AddPath}$(r,v,x)$
    our algorithm first identifies the clusters $P = \{ C_i\}$ that make up the path
    decomposition for $v$. For each such cluster $C_i$, it adds $x$ to $p_+(C_i)$. It then
    updates all of the affected clusters \guy{what is an affected
      cluster, this should be stated more clearly} and their ancestor clusters using the update rules above.
    By Lemma~\ref{lem:path_decomposition},
    this can be achieved by simply traversing the path between the base cluster of $u$ and the root of the RC tree. Since the RC tree has $O(\log(n))$ height
    and constant degree, this process takes $O(\log(n))$ time.
    \begin{comment}
    \begin{algorithm}[h]
    \caption{Path update algorithm}
    \label{alg:path_update}
    \begin{algorithmic}[1]
    \Procedure{AddPath}{$v$ : \algtype{vertex}, $x$ : \algtype{number}}
    \State \alglocal{} $P$ = \textproc{PathDecomposition}($v$)
    \For{\algeach{} \algtype{cluster} $C$ \algin{} $P$}
    \State $p_+(C)$ \algassign{} $p_+(C) + x$
    \EndFor
    \For{\algeach{} \algtype{cluster} $C$ \algin{} $P\ \cup$ \textproc{Ancestors}($P$) in bottom-up order}
    \State \textproc{UpdateCluster}($C$)
    \EndFor
    \EndProcedure
    \State
    \Procedure{UpdateCluster}{$C$ : \algtype{cluster}}
    \If{$C = \{ e \}$ \algis{} a \algtype{binary} leaf cluster}
    \State $p_{\min}(C)$ \algassign{} $w(e) + p_+(C)$
    \State $w_{\min}(C)$ \algassign{} $p_{\min}(C)$
    \Else
    \If{$C$ \algis{} a \algtype{binary cluster}}
    \State $p_{\min}(C)$ \algassign{} $\min(p_{\min}(\textproc{Top}(C)), p_{\min}(\textproc{Bot}(C))) + p_+(C)$
    \State $w_{\min}(C) = \min(p_{\min}(C), \min_{c \in \textproc{Children}(C)} w_{\min}(c))$
    \Else
    \State $w_{\min}(C) = \min_{c \in \textproc{Children}(C)} w_{\min}(c)$
    \EndIf
    \EndIf
    \EndProcedure
    \end{algorithmic}
    \end{algorithm}
    \end{comment}

\guy{This seems like a waste of space.  lets define lazy weights from
  the start.}    
    We must note that this algorithm does not actually fully update the augmented values in the RC tree. To faithfully maintain
    the values of $p_{\min}$, an update might have to process $\Theta(n)$ nodes, since the weights of the binary children of the path
    decomposition, and their binary children and so on would have to be updated. To overcome this incompleteness, the remaining updates
    are performed \emph{lazily} using the $p_+$ values. Specifically, the query algorithms must exploit the following fact:
    
\guy{lets give a notation for actual weight, as opposed to lazy weight
  instead of the vague ``true''.}
    \begin{lemma}\label{lem:true_p_val}
      After performing a sequence of updates, for a binary cluster $C$ the ``true'' value of $p_{\min}(C)$ is given by
      \begin{equation}
      p_{\min}(C) + \sum_{b \in B} p_+(b),
      \end{equation}
      where $B$ is the contiguous sequence of $C$'s immediate ancestors that are binary clusters (i.e.\ the list of $C$'s ancestors before the first unary ancestor).
    \end{lemma}
    
    \paragraph{Subtree queries.} Given a vertex $v$, a subtree query
    aims to determine the lightest edge in the subtree rooted at
    $v$. To achieve this, the algorithm computes the clusters $S = \{
    C_i \}$ that make up the subtree decomposition of $v$. The
    algorithm cannot simply return the minimum value of $w_{\min}(C_i)$
    since
    this does not account for the $p_+$ values. To account for this,
    owing to Lemma~\ref{lem:true_p_val}, the algorithm wants to
    compute, for each binary cluster $C$ in the decomposition, the
    value of $\sum_{b \in B_C} p_+(b)$. Doing this separately for each
    cluster could lead to a runtime of $O(\log^2(n))$ since each
    cluster has $O(\log(n))$ ancestors, but owing to
    Lemma~\ref{lem:subtree-decomposition}, these
    values can be computed for all of the clusters in a single top-down
    traversal from the root cluster to the base cluster of $v$, by aggregating $p_+$ for
    each contiguous chunk of binary clusters along the path and
    sending the values to their binary children. The answer to the query is then the minimum of the minimum value of $w_{\min}(C_i)$ for each cluster in the decomposition and the corrected value (Lemma~\ref{lem:true_p_val}) of $p_{\min}(C_i)$ for each binary cluster in the decomposition. By Lemma~\ref{lem:subtree-decomposition}, this process takes $O(\log(n))$ time w.h.p.
    
    \begin{comment}
    \begin{algorithm}[h]
    \caption{Subtree queries}
    \label{alg:subtree-query}
    \begin{algorithmic}[1]
    \Procedure{QuerySubtree}{$v$ : \algtype{vertex}}
    \State \alglocal{} S \algassign{} \textproc{SubtreeDecomposition}($v$)
    \State \alglocal{} $p_\text{extra}(C)$ \algassign{} $0$ for each $C \in \textproc{Ancestors}(v)$
    \For{\algeach{} \algtype{cluster} $C$ in \textproc{Ancestors}($v$) in top-down order}
    \If{$C$ \algis{} a \algtype{binary cluster}}
    \For{\algeach{} \algtype{binary cluster} $B$ \algin{} \textproc{BinaryChildren}($C$)}
    \State $p_{\text{extra}}(B)$ \algassign{} $p_{\text{extra}}(C)$ + $p_+(C)$
    \EndFor
    \EndIf
    \EndFor
    \alglocal{} answer \algassign{} $\infty$
    \For{\algeach{} \algtype{cluster} $C$ \algin{} $S$}
    \State answer \algassign{} $\min(\text{answer}, w_{\min}(C))$
    \If{$C$ \algis{} a \algtype{binary cluster}}
    \State answer \algassign{} $\min(\text{answer}, p_{\min}(C) + p_{\text{extra}}(C))$
    \EndIf
    \EndFor
    \State \algreturn{} answer
    \EndProcedure
    \end{algorithmic}
    \end{algorithm}
    \end{comment}
    
    \paragraph{Edge queries.} An edge query aims to compute, for a given edge $e$, the weight of the edge $e$. To compute this, the algorithm uses Lemma~\ref{lem:true_p_val}  and determines the $O(\log(n))$ binary clusters $\{ C_i \}$ that contain $e$ on their cluster path. The answer is then $p_{\min}(\{ e \}) + \sum p_+(C_i)$. Since the RC tree has height $O(\log(n))$, this takes $O(\log(n))$ time w.h.p.
    
    \begin{comment}
    \begin{algorithm}[h]
    \caption{Edge queries}
    \label{alg:edge-query}
    \begin{algorithmic}[1]
    \Procedure{QueryEdge}{$e = (u,v)$ : \algtype{edge}}
    \State \alglocal{} $C$ \algassign{} \textproc{Cluster}($\{ e \}$)
    \State \alglocal{} answer \algassign{} $p_{\min}(C)$
    \While{\textproc{Parent}($C$) is a \algtype{binary cluster}}
    \State $C$ \algassign{} \textproc{Parent}($C$)
    \State answer \algassign{} answer + $p_+(C)$
    \EndWhile
    \State \algreturn{} answer
    \EndProcedure
    \end{algorithmic}
    \end{algorithm}
    \end{comment}
    
    \begin{comment}
    \paragraph{Batch-dynamic subtree queries with path updates}
    
    We can also consider a batch-dynamic version of the problem. The goal is to support the following operations in low depth.
    
    \begin{itemize}[leftmargin=*]
      \item \textproc{BatchAddPath}($U = \{ (u_i, v_i, x_i) \}$): For each $(u_i, v_i, x_i)$, adds $x_i$ to the weight of all edges from $u_i$ to $v_i$
      \item \textproc{BatchQuerySubtree}($Q = \{ v_i \}$): Returns, for each $v_i$, the lightest edge in the subtree rooted at $v_i$
      \item \textproc{BatchQueryEdge}($Q = \{ e_i \})$): Returns, for each edge $e_i$, the weight of $e_i$
    \end{itemize}
    
    \noindent In Appendix~\ref{sec:batchtrees}, we prove the following theorem.
    
    \begin{theorem}\label{thm:batch-dynamic}
      There exists a parallel data structure that maintains a dynamic tree and supports the operations \textproc{BatchAddPath}, \textproc{BatchQuerySubtree}, and \textproc{BatchQueryEdge} in $O(k \log(1+n/k))$ work and $O(\log(n))$ depth, where $k$ is the batch size of the operation.
    \end{theorem}
    \end{comment}
    
    
  


==> querypath.tex <==

\section{Additional Mixed Tree Operations}\label{sec:additional-tree-ops}

We describe a simple RC implementation of \queryEdge{} and \queryPath' in Algorithm~\ref{alg:pathupdate2}. For \queryPath'{} the node $v$ must
be the representative node of an ancestor of $u$ in the RC tree.   It maintains $m$, the minimum off cluster path, $t$, the minimum on cluster path above where the path from $u$ meets the cluster path, and $b$, the minimum on cluster path below that point. Once $v$ is found it picks one of $b$ or $t$ depending on which side $v$ is, or neither if a unary cluster.
If a binary cluster it then needs to continue up the tree to add in the additional weights for binary clusters.

  \begin{algorithm}[H]
    \begin{algorithmic}[1]
    \small
\Procedure{\queryEdge}{$e$}
  \State $w \la w(e)$
  \State $x \la e$; $p \la \ra{x}{p}$
  \While{binary $p$}
    \If{$x = \ra{p}{t}$}
      \State $w \la w + \ra{\ra{p}{b}}{w} + \ra{\ra{p}{v}}{w} + \sum_{u \in \raa{p}{U}} \ra{u}{w}$
    \EndIf
    \State $x \la p$; $p \la \ra{x}{p}$
  \EndWhile
  \State return $w + \ra{\ra{p}{v}}{w} + \sum_{u \in \raa{p}{U}} \ra{u}{w}$
\EndProcedure
\Procedure{\queryPath'}{$u,v$}
  \State $m \la \infty$; $t \la \infty$; $b \la \infty$
  \State $x \la u$;  $p \la \ra{x}{p}$
  \While{not $\ra{p}{v} = v$}
    \State $w' \la \ra{\ra{p}{v}}{w} + \sum_{u \in \raa{p}{U}} \ra{u}{w}$
    \If{unary $p$}
       \If{$x = \ra{p}{t}$} $m \la \min(t + w', m)$
       \Else~$m \la\min(\ra{\ra{p}{t}}{l} + w', m)$
       \EndIf
       \State $t \la \infty$; $b \la \infty$;
     \Else
       \State $w' \la w' + \ra{\ra{p}{b}}{w}$
       \If{$x = \ra{p}{t}$} $t \la t + w'$; $b \la \min(b, \ra{\ra{p}{b}}{l})$
       \ElsIf{$x = \ra{p}{b}$} $t \la \min(\ra{\ra{p}{t}}{l} + w', t)$
       \Else~$t \la \ra{\ra{p}{t}}{l} + w'$; $b \la \ra{\ra{p}{t}}{l}$
       \EndIf
     \EndIf
     \State $x \la p$; $p \la \ra{x}{p}$
  \EndWhile
  \If{$x = \ra{p}{t}$} $l \la b$
  \ElsIf{$x = \ra{p}{b}$} $l \la t$
  \Else~return $m$
  \EndIf
  \While{binary $p$}
    \State $w' \la \ra{\ra{p}{v}}{w} + \ra{\ra{p}{b}}{w} + \sum_{u \in \raa{p}{U}} \ra{u}{w}$
    \If{$(x = \ra{p}{t})$} $l \la l + w'$
    \EndIf
  \EndWhile        
  \State return $\min(m,l)$
\EndProcedure
    \end{algorithmic}
    \caption{A \simpleRC{} implementation of \queryEdge{} and \queryPath'.}
    \label{alg:pathupdate2}
  \end{algorithm}
  
  


==> sampling-binomials.tex <==
\section{Sampling Binomial Random Variables}\label{sec:binomial}
  
  Our graph sampling procedure makes use of binomial random variables. We will
  use the following results due to Farach-Colton et al.~\cite{farach2015exact}.
  
  \begin{lemma}[Farach-Colton et al.~\cite{farach2015exact}, Theorem 1]\label{lem:sample-binom}
  Given a positive integer $n$, one can sample a random variate from the
  binomial distribution $B(n, 1/2)$ in $O(1)$ time with probability $1 - 1/n^{\Omega(1)}$ and in
  expectation after $O(n^{1/2+\varepsilon})$-time preprocessing for any constant $\varepsilon > 0$, assuming
  that $O(\log(n))$ bits can be operated on in $O(1)$ time. The preprocessing can be reused for any $n' = O(n)$
  \end{lemma}
  \noindent We can also use the following reduction to sample $B(n,p)$ for arbitrary $0 \leq p \leq 1$.
  \begin{lemma}[Farach-Colton et al.~\cite{farach2015exact}, Theorem 2]
    Given an algorithm that can draw a sample from $B(n', 1/2)$ in $O(f(n))$
    time with probability $1 - 1/n^{\Omega(1)}$ and in expectation for any $n' \leq n$, then drawing a sample from $B(n', p)$ for any real p can be done in $O(f (n)\log(n))$ time with probability $1 - 1/n^{\Omega(n)}$ and in expectation, assuming each bit of p can be obtained in $O(1)$ time
  \end{lemma}
   \noindent We note, importantly, that the model used by Farach-Colton et al.\ assumes that random $\Theta(\log(n))$-size words can be generated in constant time. Since we only assume that we can generate random bits in constant time, we will have to account for this with an extra $O(\log(n))$ factor in the work where appropriate. Note that this does not negatively affect the depth since we can pregenerate as many random words as we anticipate needing, all in parallel at the beginning of our algorithm. Lastly, we also remark that although it might not be clear in their definition, the constants in the algorithm can be configured to control the constant in the $\Omega(1)$ term in the probability, and therefore their algorithms take $O(1)$ time and $O(\log(n))$ time w.h.p.
  
  \myparagraph{Preprocessing in parallel} In order to make use of these results, we need to show that the preprocessing of Lemma~\ref{lem:sample-binom} can be parallelized. Thankfully, it is easy. The preprocessing phase consists of generating $n^{\varepsilon}$ alias tables of size $O(\sqrt{n \log(n)})$. H{\"u}bschle-Schneider and Sanders~\cite{hbschleschneider2019parallel} give a linear work, $O(\log(n))$ depth parallel algorithm for building alias tables. Building all of them in parallel means we can perform the alias table preprocessing in $O(n^{1/2+\varepsilon})$ work and $O(\log(n))$ depth. The last piece of preprocessing information that needs to be generated is a lookup table for decomposing any integer $n' = O(n)$ into a sum of a constant number of square numbers. This table construction is trivial to parallelize, and hence all preprocessing runs in $O(n^{1/2+\varepsilon})$ work and $O(\log(n))$ depth.

==> speed-up-gg.tex <==
\section{Two simple $O(m\log^2(n))$ work algorithms for $2$-respecting cuts}\label{sec:speed-up-gg} 

To demonstrate the usefulness of our mixed batch evaluation algorithm for dynamic trees, we will sketch how it can be used to produce two simple $O(m\log^2(n))$ work solutions for the minimum $2$-respecting cut problem. These both result in an $O(m\log^3(n))$ work parallel algorithm for minimum cut.

\paragraph{Parallelizing Lovett and Sandlund's algorithm.} Lovett and Sandlund~\cite{lovett2019simple} recently gave an $O(m\log^2(n))$ sequential algorithm for minimum $2$-respecting cuts. Although this does not improve on Karger's bound, it is significantly simpler than Karger's algorithm. This simplicity also makes it fairly straightforward to parallelize using our new batch evaluation algorithm. Their algorithm essentially just loops over the edges in the graph in an order determined by a heavy-light decomposition. What this means is that the graph is decomposed into chains (monotonic paths in a rooted tree) such that any path in the graph is the disjoint union of at most $O(\log(n))$ chains. The edges are then arranged in a list such that the edges of a chain are contiguous and in order from top to bottom. The goal of the algorithm while looping over each edge $e$ is to maintain for every other edge $e'$, the cost of all non-tree edges $(u,v)$ such that the $(u,v)$ path goes through $e'$ but not through $e$. Since each path consists of at most $O(\log(n))$ chains, for each non-tree edge $(u,v)$, it swaps from containing the current edge to not containing the current edge at most $O(\log(n))$ times. The algorithm can then determine which edges cause which paths to become active/inactive when visited in $O(m\log(n))$ time. It is then a simple matter of using dynamic trees to maintain the costs of every edge during the loop, and querying for the edge with the least contribution at each step. Using our batch evaluation algorithm, we can simulate the sequence of dynamic tree operations that would be performed by Lovett and Sandlund's algorithm to  obtain an $O(m \log^2(n))$ work solution that runs in $O(\log^2(n))$ depth.

\paragraph{Speeding up Geissmann and Gianinazzi's algorithm.} The algorithm of Geissmann and Gianinazzi~\cite{geissmann2018parallel} is essentially a direct parallelization of Karger's. Their important contribution was showing how to take the mixed batch of dynamic tree operations performed sequentially by Karger's algorithm, and evaluate them all at once in parallel. Specifically, they design a data structure for the monotone minimum path problem, which requires maintaining a tree $T$ subject to updates that increase the weight of all vertices along a path, and a query that asks for the minimum weight vertex on a path. Their algorithm can evaluate a sequence of $k$ operations in $O(k\log(n)(\log(n) + \log(k)) + n\log(n))$ work and $O(\log(n)(\log(n) + \log(k)))$ depth. This results in an algorithm for minimum $2$-respecting cut that runs in $O(m \log^3(n))$ work and $O(\log^2(n))$ depth. since Karger's algorithm performs $O(m\log(n))$ tree operations.
  
In Section~\ref{sec:tree-ops}, we presented our algorithm that can evaluate a sequence of dynamic tree operations consisting of subtree queries and path updates. This data structure can easily be modified to instead perform path queries rather than subtree queries; all of the major techniques are exactly the same. Since our algorithm runs $k$ operations in $O(k\log(n+k))$ work and $O(\log(n)\log(k))$ depth, plugging it into Geissmann and Gianinazzi's algorithm, and making the simple reduction from vertex weights to edge weights immediately yields an $O(m\log^2(n))$ work algorithm for minimum $2$-respecting cut that runs in $O(\log^2(n))$ depth.
